Optimal Zero-Shot Detector for Multi-Armed Attacks

This paper explores a scenario in which a malicious actor employs a multi-armed attack strategy to manipulate data samples, offering them various avenues to introduce noise into the dataset. Our central objective is to protect the data by detecting any alterations to the input. We approach this defensive strategy with utmost caution, operating in an environment where the defender possesses significantly less information compared to the attacker. Specifically, the defender is unable to utilize any data samples for training a defense model or verifying the integrity of the channel. Instead, the defender relies exclusively on a set of pre-existing detectors readily available "off the shelf". To tackle this challenge, we derive an innovative information-theoretic defense approach that optimally aggregates the decisions made by these detectors, eliminating the need for any training data. We further explore a practical use-case scenario for empirical evaluation, where the attacker possesses a pre-trained classifier and launches well-known adversarial attacks against it. Our experiments highlight the effectiveness of our proposed solution, even in scenarios that deviate from the optimal setup.

==> marco_sec1.tex <==
\textcolor{red}{To avoid comments on adaptive attacks say that it's unlikely and unrealistic and impractical to think that an attacker may know all the detectors and our final strategies is a zero-shot non trained one, directly deployed on the fly at evaluation time, so it can only be attacked to the level of its parts.}
\section{Mathematical Background}
\begin{figure}
    \centering
\resizebox{1.4\columnwidth}{!}{%
\input{plots/framework}
}
\caption[Multi-armed adversarial attacks detection]{Each sample $\x^{(k)}$ is presented to the aggregator one at a time. Note that $K, J\in\mathbb{N}$ but $J$ can be different from $K$. $\mathcal{B}er(p)$ denotes the Bernoulli distribution of parameter $p\in[0,1]$. Importantly, $\x^{(k)}\equiv\x$ when $z=0$ and  $\x^{(k)}\equiv\mathcal{A}^{(k)}_{\varepsilon, p}(\x)$ when $z=1$.}
    \label{fig:intro3}
\end{figure}
Let us consider a standard ML classification problem. Let $X$ be the random variable (r.v.) for which we have realizations $\x\in\mathcal{X}\subseteq\mathbb{R}^d$. Let $Y$ be the r.v. representing the class label, and takes values $y\in\mathcal{Y}$. Samples $(\x,y)$ are i.i.d. from the generative distribution $P_{XY}$.
The classifier can be seen as a channel representing a function $h_{\theta}:\mathcal{X}\rightarrow\mathbb{R}^{|\mathcal{Y}|}$. Generally, the output of $h_{\theta}$ is normalized to represent the posterior distribution of $p_{\widehat{Y}|X}(\cdot|\x; \theta)$.
Generally, the inference induced by the channel $h_{\theta}$ is defined as $g_{\theta}:\mathcal{X}\rightarrow\mathcal{Y}$
s.t. ${g_{\theta}(\x)\myeq \arg\max_{y\in\mathcal{Y}} p_{\widehat{Y}|X}(y|\x; \theta)}$.
We consider a scenario where a malicious actor, the attacker, intercepts the input signal $X$ before it reaches the channel, and decides whether to jam it or not according to a Bernoulli distribution $\mathcal{B}er(p)$, where $p\in[0,1]$ is the probability of jamming.
For a given signal $\x$, if the signal is jammed the channel $h_{\theta}$ will receive a corrupted input $\x'$, otherwise it will receive the original input $\x$.

A corrupted input $\x'$ is created according to a multi-armed attack system. In particular, the \textbf{attacker} has access to a set of $\mathcal{K}$ different attack strategies, \textcolor{red}{\textit{and we assume it to have black-box access to the classifier, i.e. it can query ${h_{\theta}}$} and observe its output. This is wrong, the attacker has full knowledge of the classifier $h_\theta$ (indeed we perform white-box attack on him) however it has no knowledge about the defense}.
In addition, for the sake of simplicity, we assume that the distribution over the set $\mathcal{K}$ \federica{is uniform.} Thus, we define the $k$-th attack strategy as $\mathcal{A}^{(k)}_{\varepsilon, p}: \mathcal{X}\rightarrow\mathbb{R}^d_{\varepsilon,p}$, where, with abuse of notation, $\mathbb{R}^d_{\varepsilon,p}$ represents the subset of $\mathbb{R}^d$ where the jammed samples lie, according to the general behavior of $\mathcal{A}^{(k)}_{\varepsilon, p}$ that according to its own algorithm will generate a perturbed sample $\x'\myeq\arg\max_{||\x'-\x||_p<\varepsilon}\ell(\x',\x;g_{\theta})$, where $\ell(\cdot)$ represents a loss function computed on the output of the classifier $g_{\theta}$, for the perturbed sample $\x'$, and the original sample $\x$.
\federica{For instance $\ell$ can be the \textit{Adversarial Cross Entropy loss} (ACE)~\cite{SzegedyZSBEGF13,MadryMSTV2018ICLR}, or the \textit{Kullback-Leibler divergence} (KL), or the \textit{Fisher-Rao objective} (FR)~\cite{PicotMBLBAP2022TPAMI} or the \textit{Gini Impurity score} (Gini)~\cite{GraneseRGPP2021NeurIPS}.}

\federica{I would add here the set $\mathcal{M}$, therefore the first part of section 2.1. in order to conclude 'the attacker' section}.

\federica{Here I would start a new subsection about the defender, therefore until the end of section 2.1}
Furthermore, we assume that the \textbf{defender} has no access to the model \textcolor{red}{The defender has access to the output of the model}, no access to any distribution for data sampling, and therefore it cannot robustly re-train the classifier or certify it. Finally, the defender has access only to pre-trained detectors that are given by a third party and are also not certifiable, due to the impossibility of collecting new samples\footnote{Notice that this is an interesting situation since it reduces the amount of information directly available to the defender, and therefore limits its capabilities. On the other hand, the literature on this topic proposes a rich body of detectors that can be used off the shelf.}.

In the following, we investigate how the defender must proceed to aggregate these detectors in the best possible way. It turns out that, in case there exists a detector able to distinguish between the original samples and the samples corrupted by a certain $\mathcal{A}^{(k)}_{\varepsilon, p}, \forall k\in\mathcal K$, there exists an optimal closed form solution for the aggregation of the detectors. Otherwise, in case a subset of attacks $\mathcal{K'}\subset\mathcal K$ is detected by the detectors available for the defender, we can show that, under given assumption on $\dots$.

\federica{At this point I would start the new subsection with the solution to the problem i.e., section 2.2}
% $\mathcal{A}^{(k)}_{\varepsilon, p}: \mathcal{X}\rightarrow\mathbb{R}^d$, where $k\in\mathcal{K}\subseteq\mathbb{N}$, and a constraint on the amount of noise added $||\x - \mathcal{A}^{(k)}_{\varepsilon, p}(\x)||_p$, where $||\cdot||_p$ is a L$_p$-norm. 


% An attack is a function that adds noise to the input (\emph{jammer}) to induce malfunctioning in the inference process for the given channel. Provided with knowledge of $g_{\theta}$, an attack is defined as $\mathcal{A}^{(k)}_{\varepsilon, p}: \mathcal{X}\rightarrow\mathbb{R}^d$, such that $g_{\theta}\left(\x\right)\not = g_{\theta}\left(\mathcal{A}^{(k)}_{\varepsilon, p}(\x)\right)$ according to an attack algorithm indexed as $k\in\mathcal{K}\subseteq\mathbb{N}$, and a constraint on the amount of noise added $||\x - \mathcal{A}^{(k)}_{\varepsilon, p}(\x)||_p$, where $||\cdot||_p$ is a L$_p$-norm. An attacker 


% \textcolor{magenta}{
% Provided with knowledge of $g_{\theta}$, an attack is defined as $\mathcal{A}^{(k)}_{\varepsilon, p}: \mathcal{X}'\rightarrow\mathcal{X}''$, such that $g_{\theta}\left(\x\right)\not = g_{\theta}\left(\mathcal{A}^{(k)}_{\varepsilon, p}(\x)\right)$ according to an attack algorithm indexed as $k\in\mathcal{K}\subseteq\mathbb{N}$, and a constraint on the amount of noise added $||\x - \mathcal{A}^{(k)}_{\varepsilon, p}(\x)||_p$, where $||\cdot||_p$ is a L$_p$-norm. 
% Therefore we denote by $\mathcal{X}'\subset\mathcal{X}$ the subset of the \textit{original} (clean) samples of the input space and by $\mathcal{X}''\subset\mathcal{X}$ the subset if the \textit{perturbed} (noisy) samples of the input space, i.e. $\mathcal{X}'\cup\mathcal{X}''=\mathcal{X}$ and $\mathcal{X}'\cap\mathcal{X}''=\emptyset$. 
% \begin{itemize}
% \item Given $\x\in\mathcal{X}'$ the attacker will generate a new sample according to the following strategy
% $$(1 - Z)\cdot\text{id}(\x) + Z\cdot \mathcal{A}^{(k)}_{\varepsilon, p}(\x),$$
% where $Z\sim\textit{B}er(p=.5)$ and $\text{id}$ is the identity function.
% \item Given $\x\in\mathcal{X}'$, the attacker samples an input according to $p^{(k)}_{X|Z}(x|z=1)$ .... Like before. But at this point why do we define $\mathcal{A}^{(k)}_{\varepsilon, p}$?
% \end{itemize}
% }
\section{Formalization of the Problem of Detecting multi-armed Adversarial Attacks}\label{sec:math_framework}
\federica{I would incorporate this part with the one before as I described in the comments in section 1. Moreover I would not use the word 'adversarial attack' until section 3 where we present the empirical framework}
In this section, we begin by formalizing the problem of multi-armed attacks presented before. We then delve deeper into the topic of optimal detectors and demonstrate how to apply our proposed solution to practical use cases.

\subsection{Statistical model}
\label{sec:statistical_model}

 Let $\mathcal{K}$ be the countable set of indexes corresponding to each possible attack, e.g., based on various attack algorithms and loss functions. Let  $\mathcal{M}=\big\{P^{(k)}_{XZ}\,  : \, k\in\mathcal{K} \big\}$ be the set of joint probability distributions on  $\calX\times\calZ$ which are indexed with ${k,~\forall k\in\calK}$, where $\calX$ is the input (feature) space and $\calZ=\{0, 1\}$ indicates a binary space label for the adversarial example detection task. At the evaluation time,  the attacker selects an arbitrary strategy $k\in \mathcal{K}$ and then samples an input according to $p^{(k)}_{X|Z}(\x|z=1)$ which corresponds to the probability density function induced by the chosen attack $k$ where $p^{(k)}_{X|Z}(\x|z=0)= p_X(\x) $ \emph{almost surely} corresponds to the probability distribution of the natural samples. The learner is given a set of \textit{soft-detectors} models:
$$
\Q = \left\{q_{\widehat{Z}|\logit}^{(k)} \, :\, \calU \mapsto [0,1]^2  \right\}_{k\in \calK},
$$
which have possibly been trained to detect attacks according to each strategy $k\in\mathcal{K}$, e.g.,  ${q_{\widehat{Z}|\logit}^{(k)} \equiv  p_{\widehat{Z}|U}(z|\logit; \psi_k)}$ with parameters $\psi_k$ and $\logit\in\calU = \{\classifier(\x)~|~\x\in \R^d\}$ denotes the space of logits. 
The set of possible detectors $\Q$ is available to the defender. However, the specific attack chosen by the attacker at the test time is unknown. In the remainder of this section, we formally devise an optimal detector that exploits full knowledge of the set $\Q$. 

\subsection{A novel objective for detection under simultaneous attacks}
Consider a fixed input sample $\mathbf{x_0}$ and let $\mathbf{u_0}=\classifier(\mathbf{x_0})$. Clearly, the problem at hand consists in finding an optimal soft-detector  ${q}^{\star}_{\widehat{Z}|\mathbf{u_0}}$ that performs well simultaneously over all possible attacks in  $\calK$. This can be formalized as the solution to the following minimax problem: 
\begin{equation}
\mathcal{L}(\Q, \mathbf{x_0}) = \min_{{q}_{\widehat{Z}|\mathbf{u_0}}} \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[ -\log {q}_{\widehat{Z}|\mathbf{u_0}}  \right], \label{optimal-loss}
\end{equation}
which requires to solve \eqref{optimal-loss} for $\Q$ and for each given input sample $\mathbf{x_0}$. 
It is important to note that the minimization is performed over all (detectors)  distributions ${q}_{\widehat{Z}|\mathbf{u_0}}$, including elements that are not part of the set $\mathcal{Q}$. 

That being said, the objective in~\cref{optimal-loss} is not tractable computationally. To overcome this issue, we derive a surrogate (an upper bound) that can be computationally optimized. For any   arbitrary choice of  ${q}_{\widehat{Z}|\mathbf{u_0}}$, we have 
\begin{align}
  \max_{k\in\calK}\,  \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}} &\left[ -\log {q}_{\widehat{Z}|\mathbf{u_0}}  \right] \leq \nonumber\\ 
  &\underbrace{\max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[ -\log q^{(k)}_{\widehat{Z}| \mathbf{u_0}} \right]}_{=\textrm{constant term}} + \nonumber\\ &+
  \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right].  
  \label{eq-missing}
\end{align}
\begin{proof}[Proof of~\cref{eq-missing}]
\begin{align*}
&\max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[ -\log {q}_{\widehat{Z}|\mathbf{u_0}}  \right] =\\
&=
\max_{k\in\calK}\, \left[\EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[ -\log q^{(k)}_{\widehat{Z}| \mathbf{u_0}} \right] + \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right]\right]\\
&\leq \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[-\log q^{(k)}_{\widehat{Z}| \mathbf{u_0}} \right] +\\&~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right].     
\end{align*}
\end{proof}
Observe that the first term in \eqref{eq-missing} of the upper bound is constant w.r.t. the choice of  ${q}_{\widehat{Z}|\mathbf{u_0}}$ and the second term is well-known as being equivalent to the \emph{average worst-case regret}~\cite{BarronRY1998TInfT}. This upper bound provides a surrogate to our intractable objective in \eqref{optimal-loss} that can be minimized overall ${q}_{\widehat{Z}|\mathbf{u_0}}$.  We can formally state our problem as follows: 
\begin{align}
  \label{eq:minimaxProb1}
\tilde{\mathcal{L}}(\Q,\mathbf{x_0}) = &    \min_{{q}_{\widehat{Z}|\mathbf{u_0}}}\max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right]=\nonumber\\=&\min_{{q}_{\widehat{Z}|\mathbf{u_0}}}\max_{\textcolor{black}{P_{\Omega}}}\, \EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right],
\end{align}
\textcolor{black}{where the $\min$ is taken over all the possible distributions ${q}_{\widehat{Z}|\mathbf{u_0}}$;  
and $\Omega$ is a discrete random variable with $P_{\Omega}$ denoting a generic  probability  distribution whose probabilities are  $(\omega_1,\dots,\omega_{|\calK|})$, i.e., $P_{\Omega}(k)=\omega_k$;}
and $D_{\textrm{KL}}(\cdot\|\cdot)$ is the Kullback–Leibler divergence, representing the expected value of regret of ${q}_{\widehat{Z}|U}$ w.r.t. the worst-case distribution in   $\Q$. 
\begin{proof}[Proof of~\cref{eq:minimaxProb1}]
  The equality holds by noticing that 
\begin{align*}
  \max_{P_{\Omega}}&\, \EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right] \nonumber\\
  &\leq
  \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right],
\end{align*}
and moreover, 
\begin{align*}
    \max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right]& = \EE_{\bar{\Omega}}\left[D_{\textrm{KL}}\left(q^{(\bar{\Omega})}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right],
\end{align*}
by choosing the random variable $\bar{\Omega}$ with uniform probability over the set of maximizers  ${\overline{\mathcal{K}}=\arg\max_{k\in\calK}\, \EE_{q^{(k)}_{\widehat{Z}| \mathbf{u_0}}}\left[\log\left(\frac{q^{(k)}_{\widehat{Z}|\mathbf{u_0}}}{{q}_{\widehat{Z}|\mathbf{u_0}}}\right)\right]}$, zero otherwise. 
\end{proof}
The convexity of the KL-divergence allows us to rewrite~\cref{eq:minimaxProb1} as follows:
\begin{align}
    \label{eq:minimaxProb3}
    &\min_{{q}_{\widehat{Z}|\mathbf{u_0}}}\max_{\textcolor{black}{P_\Omega}}\EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]=\nonumber\\&=  \max_{\textcolor{black}{P_\Omega}}\min_{\widehat{q}_{\widehat{Z}|\mathbf{u_0}}}\EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]. \end{align}
\begin{proof}[Proof of~\cref{eq:minimaxProb3}]
We consider a zero-sum game with a concave-convex mapping defined on a product of convex sets. The sets of all probability distributions ${q}_{\widehat{Z}|\mathbf{u_0}}$ and $P_\Omega$ are two nonempty convex sets, bounded and finite-dimensional. On the other hand, $\big(P_\Omega,{q}_{\widehat{Z}|\mathbf{u_0}} \big)\rightarrow  \EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]$ is a concave-convex mapping, i.e., $P_\Omega\rightarrow  \EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]$  is concave and ${q}_{\widehat{Z}|\mathbf{u_0}} \rightarrow  \EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]$ is convex for every $\big(P_\Omega,{q}_{\widehat{Z}|\mathbf{u_0}} \big)$.  Then, by classical min-max theorem ~\cite{vonNeumann1928-VONZTD-2} we have that~\cref{eq:minimaxProb3} holds. 

\end{proof}
The solution to~\cref{eq:minimaxProb3} provides the optimal distribution \textcolor{black}{$P_{\Omega}^\star$}, i.e. the collection of weights $\{w_k^{\star}\}$, which leads to our soft-detector~\cite{BarronRY1998TInfT}: 
\begin{align}
    \label{eq:minimaxProb4}
 \widehat{q}^{~\star}_{\widehat{Z}|\mathbf{u_0}} = \sum_{k\in\calK}w^{\star}_k \cdot q^{(k)}_{\widehat{Z}|\mathbf{u_0}}  , \ \ \text{ with } \ \ 
 \textcolor{black}{ P_{\Omega}^\star=\arg\max_{\{\omega_k\}}I_{\mathbf{u_0}}(\Omega;\widehat{Z}), }
\end{align}
where $I_{\mathbf{u_0}}(\cdot;\cdot)$ denotes the Shannon mutual information between the random variable \textcolor{black}{$\Omega$}, distributed according to \textcolor{black}{$\{\omega_k\}$}, and the binary soft-prediction variable $\widehat{Z}$, distributed according to $q^{(k)}_{\widehat{Z}|\mathbf{u_0}} $ and  conditioned on the particular test example $\mathbf{u_0}$. 
\begin{proof}[Proof of~\cref{eq:minimaxProb4}]
% \subsection{Proof of~\cref{eq:minimaxProb4}}
It is enough to show that 
\begin{align}
\min_{\widehat{q}_{\widehat{Z}|\mathbf{u_0}}}\EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right] = I_{\mathbf{u_0}}(\Omega;\widehat{Z}), \label{eq-missing-appex}
    \end{align}
for every random variable $\Omega$ distributed according to an arbitrary probability distribution $P_{\Omega}$ and each distribution $q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}$. We begin by showing that 
\begin{align*}
\EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right] & \geq  I_{\mathbf{u_0}}(\Omega;\widehat{Z}), 
    \end{align*}
for any arbitrary distributions $P_{\Omega}$ and   $q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}$. To this end, we use the following identities: 
\begin{align}
&\EE_{\Omega}\left[D_{\textrm{KL}}\left(q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}\big \| {q}_{\widehat{Z}|\mathbf{u_0}}\right)\right]
=\EE_{\Omega}\EE_{ q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}}\left(\log\frac{q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}}{ {q}_{\widehat{Z}|\mathbf{u_0}}}\right)=\nonumber\\
&= \EE_{\Omega}\EE_{ q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}}\left(\log\frac{q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}}{P_{\widehat{Z}} }\right) + \nonumber D_{\textrm{KL}}\left( P_{\widehat{Z}}  \| {q}_{\widehat{Z}|\mathbf{u_0}} \right)=\nonumber\\
&= I_{\mathbf{u_0}}(\Omega;\widehat{Z}) + D_{\textrm{KL}}\left( P_{\widehat{Z}}  \| {q}_{\widehat{Z}|\mathbf{u_0}} \right)\geq  I_{\mathbf{u_0}}(\Omega;\widehat{Z}), \label{eq-missing-appex-B}
\end{align}
where $P_{\widehat{Z}}$ denotes the marginal distribution of $q^{(\Omega)}_{\widehat{Z}|\mathbf{u_0}}$ w.r.t. $P_{\Omega}$ and the last inequality follows since the KL divergence is positive. Finally, it is easy to check that by selecting $ {q}_{\widehat{Z}|\mathbf{u_0}} = P_{\widehat{Z}} $ the lower bound in \eqref{eq-missing-appex-B} is achieved which proves the identity in expression \eqref{eq-missing-appex}. By taking the maximum overall probability distributions  $P_{\Omega}$ at both sides of expression \eqref{eq-missing-appex} the claim follows. 
% The full derivation is provided in~\cref{app:math_framework}.
\end{proof}

\noindent\textbf{From theory to our practical detector.} According to our derivation in~\cref{eq:minimaxProb4}, the optimal detector turns out to be given by a  mixture of the $|\calK|$ detectors belonging to the class $\Q$, with weights carefully optimized to maximize the mutual information between $\Omega$ and the predicted variable $\widehat{Z}$ for each detector in the class $\Q$. Using this key ingredient, it is straightforward to devise our optimal detector. 

\begin{definition}
\label{def:salad}
For any $0\leq\gamma\leq1$ and a given $\mathbf{x_0} \in\calX $, let us define the following detector $\textsc{D}:\mathbb{R}^d\rightarrow\{0, 1\}$:  
\begin{align}
\textsc{d}(\x_0)\myeq \mathds{1} \left[ {q}^{~\star}_{\widehat{Z}|\mathbf{u_0}}(\hat{z}=1|\classifier(\mathbf{x_0}))>\gamma \right],
\label{eq:salad}
\end{align}
where $\mathds{1} \left[\cdot\right]$ is the indicator function.
\end{definition}

\noindent\textbf{On the optimization of~\cref{eq:minimaxProb4}}. \federica{We implement the well-known \textit{Blahut–Arimoto algorithm}~\cite{Arimoto72}, an iterative algorithm for finding the capacity of a channel. Further details can be found in~\cref{app:optimization}}

==> plots/framework.tex <==

    
    \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
    % \fbox{
    \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
    %Straight Lines [id:da007786513349730795] (vertical line from Ber)
    \draw [color={rgb, 255:red, 0; green, 55; blue, 55 }  ,draw opacity=1]   (85.67,22.67) -- (85.67,47) ;
    \draw [shift={(85.67,47)}, rotate = -90] [fill={rgb, 255:red, 0; green, 55; blue, 55 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1 ]   (85.67,74) -- (85.67,139.99) ;
    %Straight Lines [id:da3160851740306181] (horizontal red line going inside f(x))
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1 ]   (85.67,139.99) -- (154,139.99) ;
    \draw [shift={(157,140)}, rotate = 180.18] [fill={rgb, 255:red, 108; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    %Straight Lines [id:da746487467869615] (vertical red line from Py|x to f(x))
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1 ]   (204.31,74) -- (204.31,111.67) ;
    \draw [shift={(204.33,118.67)}, rotate = 269.51] [fill={rgb, 255:red, 108; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    
    %Straight Lines [id:da6478317272567944] (horizontal red line Y hat) eccoo
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1, style=double]   (210.33,192.98) -- (325.74,192.98) ;
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1,style=double]   (325.74,175.87) -- (325.74,192.98) ;
    \draw [shift={(325.74,173.87)}, rotate = 90] [fill={rgb, 255:red, 108; green, 2; blue, 27 }  ,fill opacity=1][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    
    \draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1]   (325.74,90.87) -- (325.74,70.87) ;
    \draw [shift={(325.74,90.87)}, rotate = -90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    \draw (330.74,62.87) node    {$\gamma\in\mathbb{R}$};

    
    %Straight Lines [id:da1015283409397092] (vertical red line from f(x))
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=1, style=double]   (210.33,143.67) -- (210.33,192.98) ;
    %Straight Lines [id:da34809150153720014] (horziontal line Y_i hat)
    \draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0 ]   (254.33,140.01) -- (333,140.01) ;
    \draw [shift={(336,140)}, rotate = 179.76] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    %Straight Lines [id:da62535313665729] (horizontal red line out from Y)
    \draw [color={rgb, 255:red, 108; green, 2; blue, 27 }  ,draw opacity=0]   (205,100.98) -- (333,100.98) ;
    \draw [shift={(336,101)}, rotate = 180.45] [fill={rgb, 255:red, 108; green, 2; blue, 27 }  ,fill opacity=0 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    %Straight Lines [id:da013460956617746378] (vertical line from Y_i 1)
    \draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0 ]   (285.33,61.33) -- (285.33,100) ;
    %Straight Lines [id:da6892699350520812] (vertical line from Y_i 2)
    \draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0 ]   (285.33,102) -- (285.33,121.67) ;

     % k-----
    \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (160.91,-6) -- (259.91,-6) -- (259.91,73.2) -- (160.91,73.2) -- cycle  ;
    \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (160.91,47.2) -- (259.91,47.2) -- (259.91,73.2) -- (160.91,73.2) -- cycle  ;
    \draw (210.91,60.2) node    {$p^{(K)}_{X|Z}(\x|z)$};

    \draw  [fill={rgb, 255:red, 0; green, 0; blue, 155 },draw opacity=0  ,fill opacity=0.25 ]  (180.91,-3.2) -- (239.91,-3.2) -- (239.91,23.2) -- (180.91,23.2) -- cycle  ;
    \draw (210.91,10.2) node    {$\mathcal{B}er(p)$};
    \draw (222.91,33.2) node    [font=\small,color={rgb, 255:red, 0; green, 55; blue, 55 }  ,opacity=1 ]{$Z$};

    \draw [color={rgb, 255:red, 0; green, 55; blue, 55 }  ,draw opacity=1 ]   (210.67,22.67) -- (210.67,47) ;
    \draw [shift={(210.67,47)}, rotate = -90] [fill={rgb, 255:red, 0; green, 55; blue, 55 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;


    %____________
    % Text Node
    \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (35.91,-6) -- (134.91,-6) -- (134.91,73.2) -- (35.91,73.2) -- cycle  ;
    \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (35.91,47.2) -- (134.91,47.2) -- (134.91,73.2) -- (35.91,73.2) -- cycle  ;
    \draw (85.91,60.2) node    {$p^{(1)}_{X|Z}(\x|z)$};
    % Text Node
    % \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (35.91,107.2) -- (134.91,107.2) -- (134.91,133.2) -- (35.91,133.2) -- cycle  ;
    % \draw (85.91,120.2) node    {$P_{X|Z}(x|z=1)$};

    \draw  [fill={rgb, 255:red, 0; green, 0; blue, 155 },draw opacity=0  ,fill opacity=0.25 ]  (55.91,-3.2) -- (114.91,-3.2) -- (114.91,23.2) -- (55.91,23.2) -- cycle  ;
    \draw (85.91,10.2) node    {$\mathcal{B}er(p)$};
    \draw (97.91,33.2) node    [font=\small,color={rgb, 255:red, 0; green, 55; blue, 55 }  ,opacity=1 ]{$Z$};
    %______________



    
    % Text Node
    % \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.08, draw opacity=0 ]  (182.15,47.86) -- (255.15,47.86) -- (255.15,73.86) -- (182.15,73.86) -- cycle  ;
    % \draw (218.65,60.86)[opacity=0] node    {$p_{Y|X}(y|x)$};
    % Text Node
    \draw  [fill={rgb, 255:red, 155; green, 0; blue, 155 }  ,fill opacity=0.15 ]  (157.66,118.87) -- (253.66,118.87) -- (253.66,142.87) -- (157.66,142.87) -- cycle  ;
    \draw (205.66,130.87) node {$h_{\theta}$}  ; 
    %{$p_{\widehat{Y}|X}(\cdot|\x;\theta)$};
    % Text Node
    % \draw (144.83,53.56) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=0 ]  {$\x_{i}$};
    % % Text Node
    % \draw (287.4,53.86) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=0 ]  {$y_{i}$};
    % % Text Node
    \draw (120.67,132) node  [font=\small,color={rgb, 255:red, 108; green, 2; blue, 27 }  ,opacity=1 ]  {$\x^{(1)}$};
    % Text Node
    \draw (224.17,94.33) node  [font=\small,color={rgb, 255:red, 108; green, 2; blue, 27 }  ,opacity=1 ]  {$\x^{(K)}$};
    % Text Node
    \draw (80.17,100.17) node   [align=left] {\begin{minipage}[lt]{85.61pt}\setlength\topsep{0pt}
    \scriptsize
    % \begin{align*}
    %     \text{\scriptsize Nature:} & ~~~~\text{\scriptsize Attacker:}\\
    %     z=0 &~~~~~z=1
    % \end{align*}
    % {\ Nature:~~~~Attacker:\\$Z=0$~~~~$Z=1$}
    \end{minipage}};
    % \draw (86.17,146.17) node   [align=left] {\begin{minipage}[lt]{25.61pt}\setlength\topsep{0pt}
    % {\scriptsize Attacker}
    % \end{minipage}};
    % Text Node
    % \draw (228.5,32.83) node   [align=left, opacity=0] {\begin{minipage}[lt]{25.61pt}\setlength\topsep{0pt}
    % {\scriptsize Object}
    % \end{minipage}};
    % Text Node
    \draw (270.17,182) node   [align=left, color={rgb, 255:red, 108; green, 2; blue, 27 }] {
    \begin{minipage}[lt]{100.61pt}\setlength\topsep{0pt}
    \begin{center}
    {\scriptsize $h_\theta(\x^{(1)}); \dots; h_\theta(\x^{(K)})$ }%\\{\scriptsize (hidden variables)}
    \end{center}
    \end{minipage}};
    % Text Node
    \draw (286.74,131) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=0 ]  {$\widehat{y}_{i}$};
    % Text Node
    \draw (286.74,152.67) node  [font=\small,color={rgb, 255:red, 108; green, 2; blue, 27 }  ,opacity=1 ]  {};%{$\widehat{y}$};
    % Text Node
    % \draw (371.5,104.17) node   [align=left] {\begin{minipage}[lt]{25.61pt}\setlength\topsep{0pt}
    % {\scriptsize Loss}
    % \end{minipage}};
    
    % Text Node
    \draw  [fill={rgb, 255:red, 0; green, 255; blue, 255 }  ,fill opacity=0.3 ]  (275.74,90.87) -- (375.74,90.87) -- (375.74,172.86) -- (275.74,172.86) -- cycle  ;
    \draw (326.74,130.87) node    {
    \begin{minipage}{\textwidth}
    \begin{center}
    {\footnotesize Aggregator}\\
        \{\textsc{Detector}$_1$ \\
        $\vdots$\\
        \textsc{Detector}$_J$\}\\
    \end{center}
    \end{minipage}
    };
        %Straight Lines [id:da7854853679455196] (horizontal line from Xi to f(x))
    \draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (375.75,130.87) -- (391,130.87) ;
    \draw [shift={(391,130.87)}, rotate = 181.4] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
    \draw (436.74,120.87) node    {\textsc{\textcolor{cadmiumgreen}{Natural}}};
    \draw (436.74,140.87) node    {\textsc{\textcolor{darkred}{Adversarial}}};
    \end{tikzpicture}

